Extending the Anonymity of Zcash

Although Bitcoin in its original whitepaper stated that it offers anonymous transactions, de-anonymization techniques have found otherwise. Therefore, alternative cryptocurrencies, like Dash, Monero, and Zcash, were developed to provide better privacy. As Edward Snowden stated, "Zcash's privacy tech makes it the most interesting Bitcoin alternative (...) because the privacy properties of it are truly unique". Zcash's privacy is based on peer-reviewed cryptographic constructions, hence it is considered to provide the foundations for the best anonymity. However, even Zcash makes some privacy concessions. It does not protect users' privacy in the presence of a global adversary who is able to observe the whole network, and hence correlate the parties exchanging money, by using their network addresses. The recent empirical analysis of Zcash shows, that users often choose naive ways while performing the protocol operations, not realizing that it degrades their anonymity. In this talk, we will discuss an extension of Zcash using mix networks to enhance the privacy guarantees of users that choose to remain anonymous by tackling two major security challenges: one at the application layer of the scheme and one at its network layer.

==> fig2.tex <==
\begin{figure}[t!]\label{fig:Fig2}
    \centering
    \begin{center}
        \begin{tikzpicture}[font=\sffamily]
            \node (pool) [draw, rounded corners, thick, shape=rectangle, minimum width=1.5cm, minimum height=3cm, label={\scriptsize POOL}] {};
            \node (M) [draw, fill=white, rounded corners, shape=rectangle, left=0.5cm of pool] {M};
            \node (t1) [draw, rounded corners, shape=rectangle, left=1cm of M] {$t_1$};

            \node (t2) [draw, rounded corners, shape=rectangle, right=0.5cm of pool] {$t_2$};
            \node (t11) [draw, rounded corners, shape=rectangle, above=0.5cm of t2] {$t_1$};
            \node (dots) [shape=rectangle, below=0.1cm of t2] {$\vdots$};
            \node (t3) [draw, rounded corners, shape=rectangle, below=0.2cm of dots] {$t_n$};

            \path [->, draw, thick] (pool) -- (t11);
            \path [->, draw, thick] (pool) -- (t2);
            \path [->, draw, thick] (pool) -- (t3);

            \path [->, draw, thick] (M) -- (pool);
            \path [->, draw, thick] (t1) -- node [above] {\footnotesize com} (M);
            \path [->, draw, thick] (M) -- (t1);

            \node (p2p) [draw, dotted, thick, rounded corners, inner sep=12pt, fit=(M.mid) (pool) (t11) (t2) (t3), label=below:{\small P2P}] {};
            \node (lan) [draw, dotted, thick, rounded corners, inner sep=10pt, fit=(M.mid) (t1), label=below:{\small LAN}] {};

            \node (adv) [draw, dashed, color=red, thick, rounded corners, inner sep=15pt, fit=(p2p) (lan), label=above:{ADVERSARY}] {};
        \end{tikzpicture}
    \end{center}
\caption{Figure 2}
\end{figure}

